Ensembling Graph Predictions for AMR Parsing

In many machine learning tasks, models are trained to predict structure data such as graphs. For example, in natural language processing, it is very common to parse texts into dependency trees or abstract meaning representation (AMR) graphs. On the other hand, ensemble methods combine predictions from multiple models to create a new one that is more robust and accurate than individual predictions. In the literature, there are many ensembling techniques proposed for classification or regression problems, however, ensemble graph prediction has not been studied thoroughly. In this work, we formalize this problem as mining the largest graph that is the most supported by a collection of graph predictions. As the problem is NP-Hard, we propose an efficient heuristic algorithm to approximate the optimal solution. To validate our approach, we carried out experiments in AMR parsing problems. The experimental results demonstrate that the proposed approach can combine the strength of state-of-the-art AMR parsers to create new predictions that are more accurate than any individual models in five standard benchmark datasets.

==> refs.tex <==
\begin{thebibliography}{42}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Abadi et al(2015)]{tensorflow2015-whitepaper}
M.~Abadi {\emph{et al}}.
\newblock {TensorFlow}: Large-scale machine learning on heterogeneous systems,
  2015.
\newblock URL \url{https://www.tensorflow.org/}.
\newblock Software available from tensorflow.org.

\bibitem[Bertsekas(2011)]{Bertsekas2011}
D.P. Bertsekas.
\newblock Incremental proximal methods for large scale convex optimization.
\newblock \emph{Math. Program.}, 129\penalty0 (2):\penalty0 163--195, 2011.

\bibitem[Bottou(2009)]{bottou2009curiously}
L.~Bottou.
\newblock Curiously fast convergence of some stochastic gradient descent
  algorithms.
\newblock 2009.

\bibitem[Bottou(2012)]{bottou2012stochastic}
L.~Bottou.
\newblock Stochastic gradient descent tricks.
\newblock In \emph{Neural networks: Tricks of the trade}, pages 421--436.
  Springer, 2012.

\bibitem[Bottou et~al.(2018)Bottou, Curtis, and Nocedal]{Bottou2018}
L.~Bottou, F.~E. Curtis, and J.~Nocedal.
\newblock {O}ptimization {M}ethods for {L}arge-{S}cale {M}achine {L}earning.
\newblock \emph{SIAM Rev.}, 60\penalty0 (2):\penalty0 223--311, 2018.

\bibitem[Chang and Lin(2011)]{LIBSVM}
Chih-Chung Chang and Chih-Jen Lin.
\newblock {LIBSVM}: A library for support vector machines.
\newblock \emph{ACM Transactions on Intelligent Systems and Technology},
  2:\penalty0 27:1--27:27, 2011.
\newblock Software available at \url{http://www.csie.ntu.edu.tw/~cjlin/libsvm}.

\bibitem[Chen et~al.(2018)Chen, Liu, Sun, and Hong]{chen2018convergence}
X.~Chen, S.~Liu, R.~Sun, and M.~Hong.
\newblock On the convergence of a class of adam-type algorithms for non-convex
  optimization.
\newblock \emph{ICLR}, 2018.

\bibitem[Defazio et~al.(2014)Defazio, Bach, and Lacoste-Julien]{SAGA}
Aaron Defazio, Francis Bach, and Simon Lacoste-Julien.
\newblock Saga: A fast incremental gradient method with support for
  non-strongly convex composite objectives.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  1646--1654, 2014.

\bibitem[Dozat(2016)]{dozat2016incorporating}
T.~Dozat.
\newblock Incorporating nesterov momentum into {ADAM}.
\newblock \emph{ICLRWorkshop}, 1:\penalty0 2013–--2016, 2016.

\bibitem[Duchi et~al.(2011)Duchi, Hazan, and Singer]{AdaGrad}
John Duchi, Elad Hazan, and Yoram Singer.
\newblock Adaptive subgradient methods for online learning and stochastic
  optimization.
\newblock \emph{Journal of Machine Learning Research}, 12:\penalty0 2121--2159,
  2011.

\bibitem[Ghadimi and Lan(2013)]{ghadimi2013stochastic}
S.~Ghadimi and G.~Lan.
\newblock Stochastic first-and zeroth-order methods for nonconvex stochastic
  programming.
\newblock \emph{SIAM J. Optim.}, 23\penalty0 (4):\penalty0 2341--2368, 2013.

\bibitem[G{\"u}rb{\"u}zbalaban et~al.(2015)G{\"u}rb{\"u}zbalaban, Ozdaglar, and
  Parrilo]{gurbuzbalaban2015random}
Mert G{\"u}rb{\"u}zbalaban, Asu Ozdaglar, and Pablo Parrilo.
\newblock Why random reshuffling beats stochastic gradient descent.
\newblock \emph{arXiv preprint arXiv:1510.08560}, 2015.

\bibitem[HaoChen and Sra(2018)]{haochen2018random}
Jeffery~Z HaoChen and Suvrit Sra.
\newblock Random shuffling beats sgd after finite epochs.
\newblock \emph{arXiv preprint arXiv:1806.10077}, 2018.

\bibitem[Johnson and Zhang(2013)]{SVRG}
Rie Johnson and Tong Zhang.
\newblock Accelerating stochastic gradient descent using predictive variance
  reduction.
\newblock In \emph{NIPS}, pages 315--323, 2013.

\bibitem[Kingma and Ba(2014)]{Kingma2014}
D.~P. Kingma and J.~Ba.
\newblock {ADAM}: {A} {M}ethod for {S}tochastic {O}ptimization.
\newblock \emph{Proceedings of the 3rd International Conference on Learning
  Representations (ICLR)}, abs/1412.6980, 2014.

\bibitem[Krizhevsky and Hinton(2009)]{CIFAR10}
Alex Krizhevsky and Geoffrey Hinton.
\newblock Learning multiple layers of features from tiny images.
\newblock Technical report, Citeseer, 2009.

\bibitem[Le~Roux et~al.(2012)Le~Roux, Schmidt, and Bach]{SAG}
Nicolas Le~Roux, Mark Schmidt, and Francis Bach.
\newblock A stochastic gradient method with an exponential convergence rate for
  finite training sets.
\newblock In \emph{NIPS}, pages 2663--2671, 2012.

\bibitem[LeCun et~al.(1998)LeCun, Bottou, Bengio, and Haffner]{MNIST}
Yann LeCun, L{\'e}on Bottou, Yoshua Bengio, and Patrick Haffner.
\newblock Gradient-based learning applied to document recognition.
\newblock \emph{Proceedings of the IEEE}, 86\penalty0 (11):\penalty0
  2278--2324, 1998.

\bibitem[Li et~al.(2020)Li, Zhuang, and Orabona]{li2020exponential}
L.~Li, Z.~Zhuang, and F.~Orabona.
\newblock Exponential step sizes for non-convex optimization.
\newblock \emph{arXiv preprint arXiv:2002.05273}, 2020.

\bibitem[Li et~al.(2019)Li, Zhu, So, and Lee]{li2019incremental}
X.~Li, Z.~Zhu, A.~So, and J.~D. Lee.
\newblock Incremental methods for weakly convex optimization.
\newblock \emph{arXiv preprint arXiv:1907.11687}, 2019.

\bibitem[Loshchilov and Hutter(2017)]{loshchilov10sgdr}
I.~Loshchilov and F.~Hutter.
\newblock {SGDR}: {S}tochastic gradient descent with warm restarts.
\newblock 10:\penalty0 1--16, 2017.

\bibitem[Loshchilov and Hutter(2016)]{loshchilov2016sgdr}
Ilya Loshchilov and Frank Hutter.
\newblock Sgdr: Stochastic gradient descent with warm restarts, 2016.

\bibitem[Meng et~al.(2019)Meng, Chen, Wang, Ma, and Liu]{meng2019convergence}
Q.~Meng, W.~Chen, Y.~Wang, Z.-M. Ma, and T.-Y. Liu.
\newblock Convergence analysis of distributed stochastic gradient descent with
  shuffling.
\newblock \emph{Neurocomputing}, 337:\penalty0 46--57, 2019.

\bibitem[Mishchenko et~al.(2020)Mishchenko, Khaled, and
  Richt{\'a}rik]{mishchenko2020random}
K.~Mishchenko, A.~Khaled, and P.~Richt{\'a}rik.
\newblock Random reshuffling: {S}imple analysis with vast improvements.
\newblock \emph{arXiv preprint arXiv:2006.05988}, 2020.

\bibitem[Nagaraj et~al.(2019)Nagaraj, Jain, and Netrapalli]{nagaraj2019sgd}
Dheeraj Nagaraj, Prateek Jain, and Praneeth Netrapalli.
\newblock Sgd without replacement: Sharper rates for general smooth convex
  functions.
\newblock In \emph{International Conference on Machine Learning}, pages
  4703--4711, 2019.

\bibitem[Nedi{\'c} and Bertsekas(2001)]{nedic2001convergence}
A.~Nedi{\'c} and D.~Bertsekas.
\newblock Convergence rate of incremental subgradient algorithms.
\newblock In \emph{Stochastic optimization: algorithms and applications}, pages
  223--264. Springer, 2001.

\bibitem[Nedic and Bertsekas(2001)]{nedic2001incremental}
A.~Nedic and D.~P. Bertsekas.
\newblock Incremental subgradient methods for nondifferentiable optimization.
\newblock \emph{SIAM J. on Optim.}, 12\penalty0 (1):\penalty0 109--138, 2001.

\bibitem[Nesterov(1983)]{Nesterov1983}
Y.~Nesterov.
\newblock A method for unconstrained convex minimization problem with the rate
  of convergence $\mathcal{O}(1/k^2)$.
\newblock \emph{Doklady AN SSSR}, 269:\penalty0 543--547, 1983.
\newblock Translated as Soviet Math. Dokl.

\bibitem[Nesterov(2004)]{Nesterov2004}
Y.~Nesterov.
\newblock \emph{{I}ntroductory lectures on convex optimization: {A} basic
  course}, volume~87 of \emph{Applied Optimization}.
\newblock Kluwer Academic Publishers, 2004.

\bibitem[Nguyen et~al.(2017)Nguyen, Liu, Scheinberg, and
  Tak{\'a}{\v{c}}]{Nguyen2017sarah}
L.~M. Nguyen, J.~Liu, K.~Scheinberg, and M.~Tak{\'a}{\v{c}}.
\newblock {SARAH}: {A} novel method for machine learning problems using
  stochastic recursive gradient.
\newblock \emph{ICML}, 2017.

\bibitem[Nguyen et~al.(2020)Nguyen, Tran-Dinh, Phan, Nguyen, and van
  Dijk]{nguyen2020unified}
L.~M. Nguyen, Q.~Tran-Dinh, D.~T. Phan, P.~H. Nguyen, and M.~van Dijk.
\newblock A unified convergence analysis for shuffling-type gradient methods.
\newblock \emph{arXiv preprint arXiv:2002.08246}, 2020.

\bibitem[Nguyen et~al.(2018)Nguyen, Nguyen, van Dijk, Richtarik, Scheinberg,
  and Takac]{Nguyen2018_sgdhogwild}
Lam Nguyen, Phuong~Ha Nguyen, Marten van Dijk, Peter Richtarik, Katya
  Scheinberg, and Martin Takac.
\newblock {SGD} and {H}ogwild! convergence without the bounded gradients
  assumption.
\newblock In \emph{Proceedings of the 35th International Conference on Machine
  Learning-Volume 80}, pages 3747--3755, 2018.
  
\bibitem[Nguyen et~al.(2019{\natexlab{a}})Nguyen, Nguyen, Richt{{\'a}}rik,
  Scheinberg, Tak{{\'a}}{\v{c}}, and van Dijk]{nguyen2019newaspect}
Lam~M. Nguyen, Phuong~Ha Nguyen, Peter Richt{{\'a}}rik, Katya Scheinberg,
  Martin Tak{{\'a}}{\v{c}}, and Marten van Dijk.
\newblock New convergence aspects of stochastic gradient algorithms.
\newblock \emph{Journal of Machine Learning Research}, 20\penalty0
  (176):\penalty0 1--49, 2019{\natexlab{a}}.

\bibitem[Paszke et al (2019)]{pytorch}
A.~Paszke {\emph{et al}}.
\newblock Pytorch: An imperative style, high-performance deep learning library.
\newblock In \emph{Advances in Neural Information Processing Systems 32}, pages
  8024--8035. Curran Associates, Inc., 2019.

\bibitem[Pham et~al.(2020)Pham, Nguyen, Phan, and Tran-Dinh]{Pham2019}
N.~H. Pham, L.~M. Nguyen, D.~T. Phan, and Q.~Tran-Dinh.
\newblock {ProxSARAH}: {A}n efficient algorithmic framework for stochastic
  composite nonconvex optimization.
\newblock \emph{J. Mach. Learn. Res.}, 2020.

\bibitem[Polyak(1964)]{polyak1964some}
B.~T. Polyak.
\newblock Some methods of speeding up the convergence of iteration methods.
\newblock \emph{USSR Computational Mathematics and Mathematical Physics},
  4\penalty0 (5):\penalty0 1--17, 1964.

\bibitem[Rajput et~al.(2020)Rajput, Gupta, and
  Papailiopoulos]{rajput2020closing}
S.~Rajput, A.~Gupta, and D.~Papailiopoulos.
\newblock Closing the convergence gap of {SGD} without replacement.
\newblock \emph{arXiv preprint arXiv:2002.10400}, 2020.

\bibitem[Reddi et~al.(2016)Reddi, Hefny, Sra, P{\'{o}}czos, and
  Smola]{Reddi2016a}
Sashank~J. Reddi, Ahmed Hefny, Suvrit Sra, Barnab{\'{a}}s P{\'{o}}czos, and
  Alexander~J. Smola.
\newblock Stochastic variance reduction for nonconvex optimization.
\newblock In \emph{ICML}, pages 314--323, 2016.

\bibitem[Robbins and Monro(1951)]{RM1951}
Herbert Robbins and Sutton Monro.
\newblock A stochastic approximation method.
\newblock \emph{The Annals of Mathematical Statistics}, 22\penalty0
  (3):\penalty0 400--407, 1951.

\bibitem[Ruder(2017)]{ruder2017overview}
Sebastian Ruder.
\newblock An overview of gradient descent optimization algorithms, 2017.

\bibitem[Safran and Shamir(2018)]{Safran2019HowGoodSGDShuffling}
I.~Safran and O.~Shamir.
\newblock How good is {SGD} with random shuffling?
\newblock \emph{arXiv preprint arXiv:1908.00045}, 2018.

\bibitem[Shamir(2016)]{shamir2016without}
O.~Shamir.
\newblock Without-replacement sampling for stochastic gradient methods.
\newblock In \emph{Advances in neural information processing systems}, pages
  46--54, 2016.

\bibitem[Smith(2017)]{smith2017cyclical}
L.~N. Smith.
\newblock Cyclical learning rates for training neural networks.
\newblock In \emph{2017 IEEE Winter Conference on Applications of Computer
  Vision (WACV)}, pages 464--472. IEEE, 2017.

\bibitem[Smith(2015)]{smith2015cyclical}
Leslie~N. Smith.
\newblock Cyclical learning rates for training neural networks, 2015.

\bibitem[Tran-Dinh et~al.(2019)Tran-Dinh, Pham, Phan, and
  Nguyen]{Tran-Dinh2019a}
Q.~Tran-Dinh, N.~H. Pham, D.~T. Phan, and L.~M. Nguyen.
\newblock A hybrid stochastic optimization framework for stochastic composite
  nonconvex optimization.
\newblock \emph{Preprint: UNC-STOR 07.10.2019}, 2019.

\bibitem[Wang et~al.(2020)Wang, Nguyen, Bertozzi, Baraniuk, and
  Osher]{wang2020scheduled}
B.~Wang, T.~M. Nguyen, A.~L. Bertozzi, R.~G. Baraniuk, and S.~J. Osher.
\newblock Scheduled restart momentum for accelerated stochastic gradient
  descent.
\newblock \emph{arXiv preprint arXiv:2002.10583}, 2020.

\bibitem[Xiao et~al.(2017)Xiao, Rasul, and Vollgraf]{xiao2017fashion}
Han Xiao, Kashif Rasul, and Roland Vollgraf.
\newblock Fashion-mnist: a novel image dataset for benchmarking machine
  learning algorithms.
\newblock \emph{arXiv preprint arXiv:1708.07747}, 2017.

\bibitem[Ying et~al.(2017)Ying, Yuan, and Sayed]{ying2017convergence}
B.~Ying, K.~Yuan, and A.~H. Sayed.
\newblock Convergence of variance-reduced stochastic learning under random
  reshuffling.
\newblock \emph{arXiv preprint arXiv:1708.01383}, 2\penalty0 (3):\penalty0 6,
  2017.

\end{thebibliography}

